Balanced segmentation of CNNs for multi-TPU inference

In this paper, we propose different alternatives for convolutional neural networks (CNNs) segmentation, addressing inference processes on computing architectures composed by multiple Edge TPUs. Specifically, we compare the inference performance for a number of state-of-the-art CNN models taking as a reference inference times on one TPU and a compiler-based pipelined inference implementation as provided by the Google's Edge TPU compiler. Departing from a profiled-based segmentation strategy, we provide further refinements to balance the workload across multiple TPUs, leveraging their cooperative computing power, reducing work imbalance and alleviating the memory access bottleneck due to the limited amount of on-chip memory per TPU. The observed performance results compared with a single TPU yield superlinear speedups and accelerations up to 2.60x compared with the segmentation offered by the compiler targeting multiple TPUs.

==> CONV_4TPUs_pipeline_profiling.tex <==
\begin{table}[t]
\caption{Device memory usage in profiled segmentation of \CONV layers for 4 TPUs}%
\label{tab:CONV_4TPUs_pipeline_profiling}%
%
%\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{cc|cccc|}
%\cline{3-6}
                                                &         & \multicolumn{4}{c|}{4 TPUs w. profiling (MiB)} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}f} & \#MACs  & TPU 1    & TPU 2   & TPU 3   & TPU 4   \\ \hline
\multicolumn{1}{|c|}{292}                       & 1.26e10 & 0.82      & 0.80     & 0.80     & 0.80     \\
\multicolumn{1}{|c|}{352}                       & 1.83e10 & 1.18      & 1.16     & 1.16     & 1.16     \\
\multicolumn{1}{|c|}{412}                       & 2.51e10 & 1.61      & 1.59     & 1.59     & 1.59     \\
\multicolumn{1}{|c|}{472}                       & 3.30e10 & 2.10      & 2.08     & 2.08     & 2.08     \\
\multicolumn{1}{|c|}{532}                       & 4.19e10 & 2.66      & 2.63     & 2.63     & 2.63     \\
\multicolumn{1}{|c|}{592}                       & 5.19e10 & 3.28      & 3.26     & 3.26     & 3.26     \\
\multicolumn{1}{|c|}{652}                       & 6.29e10 & 4.00      & 3.97     & 3.97     & 3.97     \\ \hline
\end{tabular}%

\end{table}
%}

==> FC_3TPUs_pipeline_profiling.tex <==
\begin{table}[t]
%\resizebox{0.86\textwidth}{!}{%
\caption{Device memory usage in profiled segmentation of \FC layers for 3 TPUs}
\label{tab:FC_3TPUs_pipeline_profiling}
\begin{tabular}{cc|ccc|}
%\cline{3-5}
                                                &        & \multicolumn{3}{c|}{3 TPUs w. profiling (MiB)} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}n} & \#MACs & TPU 1       & TPU 2       & TPU 3       \\ \hline
\multicolumn{1}{|c|}{1140}                      & 0.40e7 & 1.32         & 1.18         & 1.32         \\
\multicolumn{1}{|c|}{1380}                      & 0.58e7 & 1.94         & 1.85         & 1.94         \\
\multicolumn{1}{|c|}{1620}                      & 0.80e7 & 2.67         & 2.57         & 2.67         \\
\multicolumn{1}{|c|}{1860}                      & 1.05e7 & 3.52         & 3.29         & 3.52         \\
\multicolumn{1}{|c|}{2100}                      & 1.33e7 & 4.36         & 4.23         & 4.36         \\
\multicolumn{1}{|c|}{2340}                      & 1.65e7 & 5.42         & 5.28         & 5.42         \\
\multicolumn{1}{|c|}{2580}                      & 2.01e7 & 6.62         & 6.46         & 6.62         \\ \hline
\end{tabular}%

\end{table}

==> mem_use_multisegment_FC.tex <==

\setlength{\tabcolsep}{2pt}

\begin{table}[t]
\caption{Memory usage of \FC models with 2 and 3 segments}
\label{tab:mem_use_multisegment_FC}

%\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{cc|cccc|cccccc|}%
%\cline{3-12}
                           &        & \multicolumn{4}{c|}{2 Edge TPUs (MiB)} & \multicolumn{6}{c|}{3 Edge TPUs (MiB)} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}n} &
  \cellcolor[HTML]{EFEFEF}\#MACs &
  \cellcolor[HTML]{EFEFEF}Dev 1 &
  \cellcolor[HTML]{EFEFEF}Dev 2 &
  Host 1 &
  Host 2 &
  Dev 1 &
  Dev 2 &
  Dev 3 &
  Host 1 &
  Host 2 &
  Host 3 \\ \hline
\multicolumn{1}{|c|}{1140} & 0.40e7 & 1.32        & 2.57        & 0        & 0          & 0.07    & 2.5     & 1.32    & 0   & 0      & 0   \\
\multicolumn{1}{|c|}{1380} & 0.58e7 & 1.94        & 3.79        & 0        & 0          & 0.09    & 3.71    & 1.94    & 0   & 0      & 0   \\
\multicolumn{1}{|c|}{1620} & 0.80e7 & 2.67        & 5.24        & 0        & 0          & 0.10    & 5.14    & 2.67    & 0   & 0      & 0   \\
\multicolumn{1}{|c|}{1860} & 1.05e7 & 3.52        & 6.93        & 0        & 0          & 0.12    & 6.81    & 3.52    & 0   & 0      & 0   \\
\multicolumn{1}{|c|}{2100} & 1.33e7 & 4.36        & 4.36        & 0        & 4.23       & 0.13    & 4.23    & 4.36    & 0   & 4.23   & 0   \\
\multicolumn{1}{|c|}{2340} & 1.65e7 & 5.43        & 5.43        & 0        & 5.28       & 0.14    & 5.28    & 5.43    & 0   & 5.28   & 0   \\
\multicolumn{1}{|c|}{2580} & 2.01e7 & 6.62        & 6.95        & 0        & 6.46       & 0.16    & 6.48    & 6.61    & 0   & 6.46   & 0   \\ \hline
\end{tabular}%
%}

\end{table}

\setlength{\tabcolsep}{6pt}

==> s4-memory_usage.tex <==
\section{Analysis of host and device memory usage}\label{sec:memory}

Motivated by the previous observations, we proceed by analyzing the executions
in terms of memory accesses. As of today, there are no profiling tools to obtain this type of
metrics; the model compiler, however, generates a compilation report that includes the amount
of host and device memory used by the Edge TPU to store the weights of the model. This
information is a good indicator of the cost associated to memory operations, as the read
operations associated to weights are the dominant operations in the inference process in terms 
of execution time (compared with the read or write of inputs and outputs, respectively, as 
the associated tensors in those operations are smaller).
%%
Additionally, the communications between host and TPU (in our case, via the PCIe bus) are a 
non-negligible bottleneck that should be reduced or avoided. In situations in which the 
model weights do not fit in device memory, the compiler will necessarily divide the 
storage of weights between device and host memory. The reduced size of the 
device memory (8 MiB) makes it common to find models that, even after quantization, cannot be 
completely stored in the device memory throughout the computation.

To support our discussion, Figure~\ref{fig:FC_CONV_time_memory_MAC} adds the amount of 
device and host 
memory used by the models deployed in the previous section.
%
%\section{External storage overhead}\label{sec:performance:overhead}
%
The memory usage perfectly explains the stepped behavior of the inference time. At each step, the device memory usage increases progressively until it reaches the available memory (8 MiB). Then, it drops sharply coinciding with an increase of host memory usage. This happens when part of the model cannot be stored on the device and starts being stored on the host. The overhead of loading these weights from the host causes the increase in inference time.

The host memory usage occurs in abrupt steps because the neural layer is the minimum storage unit: the Edge TPU compiler stores all the weights of a layer in the same memory. Theoretically, the tensors could be divided to store only the strictly necessary part of the model on the host; the compiler, however, proceeds by storing complete tensors, presumably for a simpler weight management. Their solution should perform the same number of memory copies than a storage scheme with a finer granularity, but with more data in each one. 
%\textcolor{red}{Esta ultima frase no se acaba de entender, aunque la he tratado de reescribir.}

Table~\ref{tab:FC_mem_steps} reveals that the host memory usage becomes approximately half of device memory usage for \FC layers after the first step. The reason is that one of the three large layers of the model starts to be saved on the host and there are only two large layers left on the device (there are three hidden layers with $n^2$ weights that make the $64n$ weights of the first layer and the $10n$ weights of the output layer insignificant). Similarly, a second large layer is stored on the host after the second step leaving only one big layer on the device (thus host memory usage is about twice that of device memory). Table~\ref{tab:CONV_mem_steps} reports similar qualitative results for \CONV models, which in our setup are composed by four large layers (all except the first one, which instead of $f$ input channels receives only 3).

\input{ExternalStorageOverhead/steps_FC}

\input{ExternalStorageOverhead/steps_CONV}

%\input{Tables/ExternalStorageOverhead/steps_fused}

The host memory overhead has a higher relative cost in \FC layers than in \CONV layers due to the arithmetic intensity difference between them. This is clearly seen when comparing the Edge TPU inference times with host inference times (see Figure~\ref{fig:EdgeTPUvsCPU_time}). Using the CPU, there are no communication overheads and the inference time is essentially increased by the amount of computation. For the \FC layers, we observe that the time difference between steps ($\sim$ 10 ms) is significantly higher than the CPU time of the slower models ($\sim$ 3 ms). In contrast, the time difference between steps for \CONV layers is negligible compared to the inference times on our CPU (especially if we limit the execution to a few cores). The Edge TPU stands out in these layers as the computation has a higher relative weight versus memory accesses, so the advantages of the systolic array versus more general processing are more noticeable. The difference is huge even though we are facing a low-end device against a high-end CPU.


==> stages_times.tex <==
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\definecolor{my_red}{RGB}{200,0,0} 
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{}
\label{tab:stages_times}
\begin{tabular}{l|ll|}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}Model} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Compiler segmentation stages times (ms)} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Our segmentation stages times (ms)} \\ \hline
\multicolumn{1}{|l|}{Xception}      & \multicolumn{1}{l|}{\textcolor{my_red}{15.82}, 14.25, 9.30, 2.33}                        & {\textcolor{my_red}{11.81}, 10.32, 9,74, 10.06}                      \\
\multicolumn{1}{|l|}{ResNet50}      & \multicolumn{1}{l|}{{\textcolor{my_red}{7.57}, 4.53, 4.63, 3.39}}                          & {4.76, \textcolor{my_red}{5.36}, 5.12, 5.05}                         \\
\multicolumn{1}{|l|}{ResNet50V2}    & \multicolumn{1}{l|}{{\textcolor{my_red}{8.07}, 7.11, 3.89, 2.71}}                          & {5.90, 5.34, \textcolor{my_red}{6.06}, 5.31}                         \\
\multicolumn{1}{|l|}{ResNet101}     & \multicolumn{1}{l|}{{4.58, \textcolor{my_red}{11.03}, 3.49, 2.96, 4.67, 5.40}}              & {5.05, 5.36, 4.95, \textcolor{my_red}{5.41}, 5.33, 5.21}             \\
\multicolumn{1}{|l|}{ResNet101V2}   & \multicolumn{1}{l|}{{4.21, \textcolor{my_red}{11.34}, 3.20, 4.00, 3.55, 4.45}}             & {5.23, 5.06, \textcolor{my_red}{5.54}, 5.21, 5.16, 5.17}             \\
\multicolumn{1}{|l|}{ResNet152}     & \multicolumn{1}{l|}{{6.83, 3.85, 7.46, \textcolor{my_red}{12.53}, 6.43, 1.33, 2.65, 6.18}} & {5.88, 5.91, 6.06, 5.84, 5.88, \textcolor{my_red}{6.14}, 5.76, 6.03} \\
\multicolumn{1}{|l|}{ResNet152V2}   & \multicolumn{1}{l|}{{\textcolor{my_red}{12.43}, 4.74, 5.38, 6.30, 6.22, 6.33, 3.58, 6.47}} & {6.31, 6.52, 6.28, \textcolor{my_red}{6.54}, 6.33, 6.41, 6.46, 6.38} \\
\multicolumn{1}{|l|}{InceptionV3}   & \multicolumn{1}{l|}{{\textcolor{my_red}{11.12}, 7.98, 4.00, 3.77}}                         & {6.18, 5.94, \textcolor{my_red}{6.65}, 6.32}                         \\
\multicolumn{1}{|l|}{InceptionV4}   & \multicolumn{1}{l|}{{10.12, 6.02, 6.01, 6.01, 4.27, \textcolor{my_red}{13.55}, 10.37}}      & {8.06, 8.15, \textcolor{my_red}{8.19}, 7.86, 8.04, 7.97, 8.13}       \\
\multicolumn{1}{|l|}{Inc.ResNetV2}  & \multicolumn{1}{l|}{{7.63, 6.66, 6.31, 3.01, 7.66, 6.83, 6.71, \textcolor{my_red}{20.71}}} & {8.19, 8.23, 7.94, 8.31, 8.14, \textcolor{my_red}{8.33}, 8.04, 8.22} \\
\multicolumn{1}{|l|}{DenseNet121}   & \multicolumn{1}{l|}{{\textcolor{my_red}{8.23}, 3.78}}                                      & {5.86, \textcolor{my_red}{5.92}}                                     \\
\multicolumn{1}{|l|}{DenseNet169}   & \multicolumn{1}{l|}{{\textcolor{my_red}{12.50}, 9.60, 4.16}}                               & {8.68, 8.74, \textcolor{my_red}{8.92}}                             \\
\multicolumn{1}{|l|}{DenseNet201}   & \multicolumn{1}{l|}{{12.82, \textcolor{my_red}{13.37}, 6.78, 4.43}}                        & {9.02, 9.41, 9.83, \textcolor{my_red}{9.46}}                        \\
\multicolumn{1}{|l|}{Eff.NetLiteB3} & \multicolumn{1}{l|}{{\textcolor{my_red}{3.74}, 3.52}}                                      & {3.65, \textcolor{my_red}{3.72}}                                     \\
\multicolumn{1}{|l|}{Eff.NetLiteB4} & \multicolumn{1}{l|}{{\textcolor{my_red}{10.14}, 9.64, 8.05}}                               & {\textcolor{my_red}{9.33}, 9.16, 9.25}                               \\ \hline
\end{tabular}
\end{table}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1/1.2}

==> steps_FC.tex <==

\begin{table}[t]
\centering
\caption{Memory usage and inference time before and after each step for \FC models}
\label{tab:FC_mem_steps}
%\resizebox{0.42\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
Step               & \#MACs   & Device (MiB) & Host (MiB) & Inf. time (ms)  \\ \hline
                    & 0.76e7 & 7.43 & 0 & 0.17  \\
\multirow{-2}{*}{1} & 0.79e7 & 5.27 & 2.63 & 7.42 \\ \hline
                    & 1.19e7 & 7.66 & 3.82 & 10.62 \\
\multirow{-2}{*}{2} & 1.24e7 & 4.04 & 8.04 & 21.83 \\ \hline
\end{tabular}%
%}

\end{table}

==> steps_fused.tex <==

\begin{table*}
\centering
\begin{subtable}{.45\linewidth}\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
Step               & \#MACs   & Device (MiB) & Host (MiB) & Inf. time (ms)  \\ \hline
                    & 0.76e7 & 7.43 & 0 & 0.17  \\
\multirow{-2}{*}{1} & 0.79e7 & 5.27 & 2.63 & 7.42 \\ \hline
                    & 1.19e7 & 7.66 & 3.82 & 10.62 \\
\multirow{-2}{*}{2} & 1.24e7 & 4.04 & 8.04 & 21.83 \\ \hline
\end{tabular}%
\caption{\FC models}
\label{tab:FC_mem_steps}
\end{subtable}
%%%
\begin{subtable}{.45\linewidth}\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
Step               & \#MACs  & Device (MiB) & Host (MiB) & Inf. time (ms) \\ \hline
                    & 2.88e10 & 6.86 & 0 & 41.34 \\
\multirow{-2}{*}{1} & 3.01e10 & 5.99 & 1.99 & 61.60 \\ \hline
                    & 3.87e10 & 6.78 & 2.25 & 69.71 \\
\multirow{-2}{*}{2} & 4.02e10 & 5.21 & 5.19 & 96.89 \\ \hline
                    & 5.89e10 & 6.98 & 6.95 & 126.41 \\
\multirow{-2}{*}{3} & 6.08e10 & 3.93 & 11.69 & 232.82 \\ \hline
\end{tabular}%
\caption{\CONV models}
\label{tab:CONV_mem_steps}
\end{subtable}
\caption{Memory usage and inference time before and after each step}
\end{table*}
